Automatic Detection, Validation and Repair of Race Conditions in Interrupt-Driven Embedded Software

Interrupt-driven programs are widely deployed in safety-critical embedded systems to perform hardware and resource dependent data operation tasks. The frequent use of interrupts in these systems can cause race conditions to occur due to interactions between application tasks and interrupt handlers (or two interrupt handlers). Numerous program analysis and testing techniques have been proposed to detect races in multithreaded programs. Little work, however, has addressed race condition problems related to hardware interrupts. In this paper, we present SDRacer, an automated framework that can detect, validate and repair race conditions in interrupt-driven embedded software. It uses a combination of static analysis and symbolic execution to generate input data for exercising the potential races. It then employs virtual platforms to dynamically validate these races by forcing the interrupts to occur at the potential racing points. Finally, it provides repair candidates to eliminate the detected races. We evaluate SDRacer on nine real-world embedded programs written in C language. The results show that SDRacer can precisely detect and successfully fix race conditions.

==> Sections/Abstract.tex <==
% !TeX root = ../bare_NDSS.tex

\begin{abstract}
Interrupt-driven programs are widely deployed in safety-critical embedded systems 
to perform hardware and resource dependent data operation tasks. 
The frequent use of interrupts in these systems can cause data races to 
occur due to interactions between application tasks and interrupt handlers. 
Numerous program analysis and testing techniques have been proposed to 
detect races between threads. Little work, however, has addressed data 
race problems related to interrupt handlers.
In this paper, we present \Name{}, an automated framework that helps 
in detecting and fixing data races  in interrupt-driven embedded software.  
It uses a combination of static analysis, symbolic execution and dynamic 
simulation to synthesize the failure-inducing data input and interrupt 
interleaving schedule. In addition,  \Name{}  can further suggests fixes 
based on the identified  data races.  We evaluate \Name{} on ?? embedded 
programs with both known and previously unknown data races. 
The results show that \Name{} precisely detects data races and that it  
successfully fixes data races without causing deadlocks or excessive 
performance degradation. The suggested fixes are of similar quality 
to those manually written by developers.
\end{abstract}


==> Sections/Background.tex <==
% !TeX root = ../bare_conf.tex

\section{Motivation and Background}
\label{sec:background}

In this section we use examples to illustrate the challenges
in detecting and fixing data races and then formally define
our problem.

\subsection{Motivating Example}
\label{sec:example}


Figure \ref{exp1} shows a code snippet from
a keyboard device driver program~\cite{X}.
This code has one application task {\tt task1}
and two interrupt handlers associated with two
hardware interrupts where irq1 has a higher priority
than irq2. There are two shared variables:
{\tt mode} and {\tt packetsNumber}.
This program contains a race condition.
Under normal execution, task1 reads the
the variable {\tt packetsNumber} and decreased its value.
However, if irq1 occurs before the variable is decremented (line~\ref{exp1:cri}),
{\tt packetsNumber} is modified and task1 reads the wrong value.
This race would cause serious system failure.

The first challenge is that testing race condition
related to interrupts requires synchronization modeling
to compute happens-before relations between concurrency events.
Embedded systems use special operations to control
interrupts, some of which may not even be recognized by
existing static and dynamic analysis techniques analysis.
For example, task1 enables the interrupt by directly
flagging an interrupt bit at the hardware level.
Failing to identify such operations would report
false positives. For example, existing techniques would falsely report that
there is a race condition between line \ref{exp1:sv1} and line \ref{exp1:sv2} on the variable
{\tt packetsNumber} even if irq is disabled in task1.
Therefore, hardware states and operations must be observed when
testing for race conditions in interrupt-driven embedded systems.

Second,  task and interrupt priorities affect happens-before relations
between concurrency events. For example,
the read of {\tt packetsNumber} at line
line~\ref{exp1:cri} and the write of {\tt packetsNumber} at line \ref{exp1:sv2} cannot race because
irq1 has a higher priority than irq2. Therefore,
existing techniques that neglect the effect of priorities
would lead to false positives.
This problem can become more complicated in the presence of nested
interrupts with different priorities.

Third, testing this code requires specific input. This race
can only be triggered when both two conditions in
the {\tt irq1\_handler} are false. Existing techniques
on testing interrupt-driven programs rely on existing inputs.

Fourth, races detected by static analysis or
dynamic analysis following random scheduling  may report
false positives. Therefore, controllability is needed
to validate whether a race detected by these techniques
are real or not.  Several existing
approaches have tried to abstract away scheduling
non-determinism in concurrent programs to achieve
greater execution control (e.g.,~\cite{Sen08}).
These approaches often control thread scheduling, but
cannot force hardware interrupts to occur at arbitrary point.

Finally, fixing interrupt-related race conditions requires
enforcing synchronization operations that specific to interrupts.
In this example, the interrupt disabling operation associated
with irq1 should be inserted before line \ref{exp1:sv1}. However, finding
the place to enable interrupt is important because long critical
section may lead to timing or performance violations.
Existing techniques on fixing thread-level concurrency faults
cannot be directly adapted to address this problem.

\lstset{
  language={[ANSI]C},
  basicstyle=\fontsize{6}{6}\ttfamily, mathescape,
  breaklines=true,
  showstringspaces=false
  }
\noindent

\begin{figure}[t]
%\centering
\footnotesize
\begin{mdframed}[roundcorner=5pt]
\vspace*{-10pt}
\begin{lstlisting}
void task1()
{
  disable_irq(2);
  if(mode)
    packetsNumber = packetsNumber - 1; (*@\label{exp1:sv1}@*)
  else
    bufferRemainCap++;
  set_irq_bit(2, 10);
}
irqreturn_t irq1_handler()
{
  if(mode)
  {
    if(packetsNumber != -1) (*@\label{exp1:read}@*)
      packetsNumber = packetsNumber + 1; (*@\label{exp1:cri}@*)
  }
}
irqreturn_t irq2_handler()
{
   packetsNumber = packetsNumber - 1; (*@\label{exp1:sv2}@*)
}

\end{lstlisting}
\vspace*{-10pt}
\end{mdframed}
\vspace*{-5pt}
\caption{\label{exp1} \textbf{\small An example of Keyboard driver}}
\normalsize
\vspace*{-5ex}
\end{figure}

\ignore{
\begin{figure}[t!]
%\centering
\footnotesize
\begin{mdframed}[roundcorner=5pt]
\vspace*{-10pt}
\begin{lstlisting}
static int data;
void task1( ) {
  init();
  enableinterrupt( );
  ...
  data = x ;
  int i = 0 ;
  while(i < MAX)
    str[data] += x ;
}
void interrupt1( )
{
  int i;
  ...
  for(; i < 10 ; ++i )
  {
    y = data ;
    readDate(y);
  }
}
\end{lstlisting}
\vspace*{-10pt}
\end{mdframed}
\vspace*{-5pt}
\caption{\label{exp2} \textbf{\small A false positive}}
\normalsize
\vspace*{-5ex}
\end{figure}
}

\subsection{Interrupt-driven Embedded Systems}
%
In embedded systems, an interrupt alerts the processor to a high-priority condition requiring
the interruption of the current code the processor is executing.
The processor responds by suspending its current activities, saving its state,
and executing a function called an interrupt handler (or an interrupt service routine, ISR)
to deal with the event. This interruption is temporary, and, after the interrupt handler
finishes, the processor resumes normal activities.

We denote an interrupt-driven program by
$P$ = {\tt Task} $\|$ {\tt ISR},
where {\tt Task} is the main program that consists
of one or more tasks (or threads) and
{\tt ISR} = $ISR_1 \| ISR_2 \| \ldots \| ISR_N$
indicates interrupt service routines. The
subscripts of ISRs indicate interrupt numbers,
with larger numbers denoting lower priorities.
Typically, $P$ receives two types of \emph{incoming data}:
command inputs as entered by users
and sensor inputs such as data received
through specific devices (e.g., a UART port).
An \emph{interrupt schedule} specifies a sequence
of interrupts occurring at specified program locations.
The input data and an interrupt schedule for $P$
together form a \emph{test case} for $P$.
In this work, we do not consider reentrant interrupts
(interrupts that can preempt themselves); these are uncommon
and used only in special situations~\cite{Regehr05}.

\wym{Change the condition of our method, i.e., now we focus on race caused by interrupt and concurrency.}
Note that races may also occur between tasks like
multi-threaded programs.
Races caused by interrupts unlike thread-level races,
an interrupt handler usually cannot be blocked unless additional interrupt
handler with higher priority preempts it, otherwise it will continue running until finished.
There is an asymmetric relationship between interrupt handlers and tasks. Namely,
the interrupt handler can preempt the task, but not vice versa.
In this work,
we focus on race conditions caused by interrupts and multi-threaded.
However, we mostly discuss race conditions caused by interrupts in this paper.

\subsection{Data Races in Interrupt-driven Programs}
%

%Similar with the formal define of data race \cite{o2003hybrid}, we present a
% definition of data race in interrupt-driven program as follows:

%%%%$e_i = MEM(m_i, a_i, t_i) \land e_i= MEM(m_j, a_j, t_j) \land t_i \neq t_i \land m_i = m_j \land (a_i = WRITE \lor a_j = WRITE) \land L_i(t_i) \cap L_j(t_j) = \emptyset$

A data race at some global variable $x$ occurs if a task or an interrupt
execution $p$ reaches an access to $x$ at a priority $m$ while $x$ also might be
accessed by some interrupt $q$ of priority $m$, where $m > n$. More formally,

\begin{center}
%$S_t \rightarrow S_i \land P_t \ne P_i\land M_t = M_i \land
%(A_i = WRITE \lor A_j = WRITE) \land (L_i(t_i) \cap L_j(t_j) = \emptyset)$
\footnotesize
$\mathit{
e_i = MEM (\alpha_i, m_i, a_i, t_i, h_i, p_i) \wedge e_i = MEM (\alpha_j, m_j,
a_j, t_j, h_j, p_j)}$
$\mathit{\wedge t_i \neq t_j \wedge m_i = m_j \wedge (a_i = WRITE \vee a_j =
WRITE)}$
$\mathit{  \wedge \neg (e_i \prec e_j) \wedge
\neg (e_j \prec e_i)
}$
\end{center}

\noindent
%In the above definition, t and i represent two functions (Usually a task and an
% ISR).
%$RaceWarning(S_t, S_i)$ denotes a potential data race at statement $S_t$ and
% $S_i$, and i preempts t.  $M_t = M_i$ denotes that they access the same memory address.
%$A_i = WRITE \lor A_j = WRITE$ shows that at least one of the two memory access
% is write.
%The last constraint represents that the two access aren't protected by the same
% lock.
%In interrupt-driven embedded systems, two ISRs with different priorities could
% also result in data race. $P_t \ne P_i$ is used to constraint the priorities of two functions.
%This is data races caused by nested interrupts.
%%%%%%%%data is consistent if isr is read, data will be inconsistent vice versa.
%
The above condition states that two events $e_i$ and $e_j$ are in race condition
if they access the same memory location without holding a happens-before
relation, they are from different tasks or interrupt handlers,
at most one event is from the task, and at least one of the accesses is a write.
MEM($\alpha$, $m_i$, $a_i$, $t_i$, $h_i$, $p_i$) denotes that
task or interrupt handler $t$ with priority $P$ performs
an access a $\in$ \{WRITE, READ\} to memory location $m$ while
in an hardware state $H$ (e.g., interrupt is enabled)
and executing the statement $\phi$.
The computation of the relation $\prec$ is done by
maintaining happens-before relations with every access.




%%%%%%%%%Data race detection for interrupt-driven programs can improve the stability of embedded systems due to the following reasons: First, compared to other common issues, data races are more harmful to embedded systems because data races are often hard to be found, difficult to be repaired. This will result in serious failures. Data races can not only affect the stability of the system, but also affect the system development efficiency, leading to project failure if they are not found until the system integration. Secondly, programming errors that are not directly related to concurrency can also be revealed by data race detecting methods. Data race is caused by incorrect or insufficient synchronization, but some bugs that are not directly related to shared memory, such as buffer overflow, use-after-free and so on, can be detected through data race detecting methods. Therefore, industry or academia pays special attention to data race in interrupt-driven programs.




\ignore{
\subsection{Symbolic Execution}
Symbolic execution is a method that analyzing inputs that cause each part of a program to execute.
Symbolic execution engine regards specific values like inputs as symbolic values rather than concrete values.
In some specific execution points, the engine tries to solve constraint combined of symbolic values.
It can provide actual values of the symbolic values if constraints are able to solve.
However, symbolic execution faces challenges like path explosion, which will unable to solve constraints.
For the example at Listing \ref{exp1}, most dynamic testing method could hardly cover the two branches
at function \emph{task2} if the variable \emph{mode} is determined by external input. In contrast,
symbolic execution could solve the constraint and generate the corresponding test cases that cover two branches.

Recently, lots of symbolic execution tools are proposed. KLEE \cite{KLEE} is a symbolic virtual
machine built on top of the LLVM compiler infrastructure. JPF \cite{JPF} is an explicit state
software model checker for Java bytecode.

\subsection{Simulation and Simics}
Simulation technical enables one computer system (called the host) to behave like another
computer system (called the guest). Typically, it enables the host system to run software
or use peripheral devices designed for the guest system.
A full-system simulator can simulate an electronic system that software from real
systems can run on the simulator without any modification.
A full-system simulator provides virtual hardware that is independent of the host computer.
The full-system simulator  supports the design, development, and testing of computer hardware
and software within a simulation framework that approximates the final application
context \cite{magnusson2002simics}. Compared with full-system simulator, an instruction set simulator
can't allows real device drivers and operating systems to be run and only supports single programs.

Simics \cite{simics15} is a full-system simulator used to run unchanged production
binaries of the target hardware at high-performance speeds.
Simics can simulate almost all of common systems such as Alpha, X86-64, IA-64, etc.
Many operating systems have been run on various varieties of the simulated hardware,
including MS-DOS, VxWorks, FreeBSD, Windows, Linux, etc.

Advantages of Simics are as follows. First, similar to other full-system simulators,
Simics provides functional and behavioral characteristics similar to those of the target
hardware system, enabling software components to be developed, verified, and tested as if
they are executing on the actual systems. Second, Simics can run, observe and control various
system behaviors without the source code. Third, Simics can add the proposed capabilities to
enable adoption without requiring much effort due to its powerful device modeling infrastructure.
Our simulation achieves observability by utilizing its abilities to monitor memory accesses
and hardware states as a program executes and report faults related to oracles; the observed
information is also used to guide controllability at certain program points.
Controllability is achieved by utilizing Simics abilities to interrupt execution
without affecting the states of the guest system. As such, engineers can manipulate
memory and buses directly to force interrupts so that they test only the locations
that have potential races. Controllability is also achieved by forcibly changing
the execution path when needed. As such, engineers can manipulate execution
paths so that they test the locations that not easily executed.
}




==> Sections/Conclusion.tex <==
% !TeX root = ../bare_conf.tex

\section{Conclusion and further work}
\label{sec:clu}
This paper presents a new data race detection method for interrupt-driven programs. This method is a combination of static analysis. symbolic execution, dynamic simulation and race fix. First, we propose a static analysis method for identifying potential data race scenarios in interrupt-driven programs. Second, symbolic execution is used to generate test cases or external inputs for different race scenarios. Then, we present a dynamic simulation approach guided by static race warnings. Thanks to system simulation tool and its system model, we can dynamically monitor system state, control execution, and confirm the results of static analysis. Finally, we automatically fix the races according to the priority of potential data races. In addition, we implement a prototype tool based on our method, and conduct a controlled experiment to demonstrate the effectiveness of our approach.

In the future, we will further improve the accuracy of static analysis and the automation of the framework, as well as to extent our approach to other types of concurrency bugs.

\section{Acknowledgment}
\label{sec:ack}
The paper was partially supported by the National Natural Science Foundation of China (No. 61321491, No.61472179).


==> Sections/Implementation.tex <==
% !TeX root = ../bare_conf.tex

\section{Implementation and Experiment}
\label{sec:imp}
\subsection{Implementation}
Our method is divided into four modules, static analysis, symbolic execution,
dynamic validation and automatical fix.
%We extend SVs detection algorithm from \cite{abdelqawy2012survey} to detect SVs.
CFGs are provided by Clang Tool \cite{Clangtool} to construct RCFGs.
In the meantime, alias analysis is performed using Steensgard’s~\cite{steensgaard1996points}
algorithm to avoid ignoring alias of shared resources.
Symbolic execution is implemented based on KLEE~\cite{KLEE} and KLEE-uClibc~\cite{KLEEuclibc}.
Since most kernel functions are not supported by KLEE and KLEE-uClibc,
we extend KLEE-uClibc to support kernel functions like \emph{request\_irq()}.
In order to support guided symbolic execution, we modify KLEE to only gather
constraints related to the paths that are generated by static analysis.
The virtual platform used for dynamic validation is provided by
Simics 4.6 \cite{simics15}. Scripts for the virtual platform used
to set breakpoints, define callback functions are written in Python.
Finally, automatic race fix are written in Python.

\subsection{Evaluation Design and Setup}
To validate the effectiveness of our approach, we designed
some experiments using our approach.
Experimental subjects: The first three subjects are real
interrupt-driven programs acquired from industry,
named module1, module2 and module3, respectively. Module1 is
a type of UART driver. Module2 is used to control the power of engine.
 Module3 is a driver for lower computer. Two experiments are from
 LDD \cite{corbet2005linux} named short and shortprint.
 The keyboard driver is a cooked program.
 The other programs are from Linux Kernel.
 All our experiments were performed on a PC with 4-core Intel Core
 CPU i5-2400 (3.10GHz) and 8GB RAM on Ubuntu Linux 12.04.
 For the simulation, the Host OS is Ubuntu 12.04 and the guest OS is 10.04.

\subsection{Result}
\label{sec:result}

\begin{table}[!t]
\centering
\caption{Experiment Results}
\begin{tabular}{|P{1.0cm}|P{0.5cm}|c|c|c|c|c|c|P{0.3cm}|P{0.3cm}|}
\hline
% TODO: explain some symbolic execution is hard to continue
Program name        & LOC   & \#I   & \#T   & \#SR  & \#Blo  & \#W   & \#S   & AR    & TR \\\hline % code mean: 1:true race, 2:AR reduced, 3:Symb reduced
module1             & 168   & 1     & 3     & 1     & 55     & 11    & 11    & 4     & 4 \\\hline % datarace
module2             & 153   & 2     & 37    & 4     & 62     & 93    & 40    & 40    & 43 \\\hline % line box:
module3             & 102   & 2     & 8     & 1     & 40     & 15    & 10    & 10    & 10 \\\hline % power
%module1             & 168   & 1     & 3     & 1     & 55     & 26    & 16    & 3     & 3 \\\hline % 22222 13322 22113 33223 33333 2
%module2             & 153   & 2     & 37    & 4     & 62     & 139   & 69    & 60    & 63 \\\hline
%line box: 139 warnings :(  . 13331 13111 33331 11333 31113 33311 13333 11133 33133 11111 33111 11331 11333 31331 11113 31111 13321 13211 32211 31133 31113 33111 3*30
%module3             & 102   & 2     & 8     & 1     & 40     & 14    & 8     & 4     & 4 \\\hline %power: . 11.13    NOTE: array[SV] = num; ignore the read access. 12112 13333 33322
short               & 704   & 5     & 18    & 20    & 315    & 127   & N/A   & 43    & 43 \\\hline %
short (EI)          & 707   & 5     & 18    & 20    & 317    & 149   & N/A   & 55    & 55 \\\hline %
shortprint          & 531   & 1     & 11    & 22    & 266    & 4     & N/A   & 1     & 1 \\\hline %
shortprint (EI)     & 530   & 1     & 11    & 22    & 266    & 14    & N/A   & 11    & 11 \\\hline %
keyboard driver     & 84    & 1     & 4     & 5     & 45     & 4     & 3     & 3     & 3 \\\hline %
% following is unable to ins module.
%pc110pad            & 179   & 1     & 3     & 5     & 46     & 7     & N/A   & 1     & 1 \\\hline
%mk712               & 219   & 1     & 6     & 4     & 56     & 10    & N/A   & 5     & 5 \\\hline
%8250                & 2659  & 1     & 22    & 8     & 457    & 17    & N/A   & 1     & 1 \\\hline %Need to review the last three results.
%serial-u16550 (EI)  & 1039  & 1     & 24    & 11    & 378    & 1     & 1     & 1     & 1 \\\hline %EI version: remove spin_lock
%mtpav   (EI)        & 785   & 1     & 17    & 9     & 293    & 2     & 2     & 2     & 2 \\\hline % leave here at 11.7
mpu401\_ uart (EI)  & 630   & 1     & 16    & 2     & 316    & 146     & 1     & 1     & 1 \\\hline
i2c-pca-isa (EI)    & 225   & 1     & 11    & 9     & 111    & 4     & 4     & 1     & 1 \\\hline % verified at 1.16
%intel\_scu \_ipc    & 675   & 1     & 16    & 7     & 215    & 5     & 5     & 4     & 2 \\\hline % Add constraint so that we can reduce a warning in free_irq.
%inport (EI)         & 199   & 1     & 5     & 3     & 37     & 7     & 1     & 1     & 1 \\\hline
mv643xx \_eth.c       & 3256  & 1     & 29    & 7    & 1076   & 16    & 10    & 10    & 10 \\\hline % 1111111111
%module2 kernel      & 104   & 2     & 3     & 1     & 20     & 61    & 40    & 40    & 43 \\\hline
%gusmax.c             & 384   & 1     & 16    & 11    & 158    & 4     & 4     & 0     & 0 \\\hline
%opl3sa2  & 630   & 1     & 17    & 1     & 316    & 1      & 1     & 1     & 1 \\\hline  % It's FP
%wss\_lib     & 2297   & 1    & 42    & 5     & 895    & 28       & N/A     & 28     & 28 \\\hline % too many warnings.
%cyclades    & 4164   & 2    & 28    & 16     & 1574    & 24       & 0     & 0     & 0 \\\hline % too many warnings.
\end{tabular}%}
\label{tableRes}
\end{table}%

Table \ref{tableRes} shows experiment results of different subjects.
\emph{\#I} means number of interrupts in programs, different interrupts have different priorities for these programs; \emph{\#T} represents
number of tasks; \emph{\#SR} represents number of SRs; \emph{\#W} means
number of warnings reported by static analysis;
\emph{\#S} represents the number of warnings remained after conducting symbolic
execution; this field also represent the number of test cases generated by
symbolic execution.
\emph{\#Blo} shows the number of blocks for each program. This field shows a part of complexity for symbolic execution.
\commentty{maybe we should also include the number of branches.} \wy{added}
The reason is due to the small scale of test cases, symbolic execution could generate all test cases
except for unreachable paths. For programs do not have external inputs or
symbolic execution can not eliminate false positives, we use \emph{N/A} to represent this situation.
Some of our test cases don't need to perform symbolic execution because their races don't depend on parameters.
However, although symbolic execution can not provide test cases for these programs,
it can eliminate false positives. Because some warnings are unable to reach due to the confliction of path constraints.
\emph{AR} means number of data race validated by simulation; and \emph{TR} represents number
of manually confirmed data races. Two program name followed
by \emph{EI} means that races in these program are manually injected.
We inject a shared variable increment operation and a decrement operation at interrupt handlers.
The error injection will not change the semantic of original programs but import new data races for these programs.

\begin{table}[!t]
\centering
\caption{Experiment Results}
\begin{tabular}{|P{1.0cm}|c|c|c|c|c|}
\hline
\multirow{2}{*}{Programs} & \multicolumn{3}{c|}{Execution Time (second)}  & \multicolumn{2}{c|}{Overhead} \\\cline{2-6}
& \tabincell{c}{Static\\Analysis} & \tabincell{c}{Symbolic\\Execution} & Sim & Sim & \tabincell{c}{Automatic\\Repair} \\\hline
% in simics make time overhead: 4400%
% note that we use klee to solve specific path.
% Simulation time is average time for real race, including test input time. Because the threshold time will affect analysis time.
% Simulation time is based on real time mode. Without VMP. The time is calculated by callback
% disable_irq overhead is depending on the irq line, 1 is higher than 10.
module1             & 0.076   & 0.228     & 1.54  & 66924\% & 81.35\%/104.51\%     \\\hline % sim time: 937970us, real time:1233us
module2             & 0.075   & 0.231     & 1.25  & 59008\% & 7.01\%/34.52\%     \\\hline %
module3             & 0.073   & 0.226     & 1.06  & 42604\% & 7.51\%/92.3\%     \\\hline % power
short               & 0.109   & 0.327     & 26.8  & 29703\% & 3.21\%/25.4\%    \\\hline %
short (EI)          & 0.106   & 0.324     & 24.13 & 28564\% & 3.14\%/26.1\%    \\\hline %
shortprint          & 0.088   & 0.313     & 21.61 & 44563\% & 4.85\%/32.4\%    \\\hline %
shortprint (EI)     & 0.091   & 0.317     & 49.3  & 42584\% & 4.56\%/33.4\%    \\\hline %
keyboard driver     & 0.073   & 0.258     & 1.65  & 89200\% & 0\%/33.33\%     \\\hline %sim time: 1.639s, real time:1652us, 3 real races take 1.65s average time.
mpu401\_ uart (EI)  & 0.088   & 0.355     & 75.2  & 24532\% & 3.75\%/15.48\%    \\\hline % KLEE report assetion if "snd_mpu401_uart_new" is analyzed. not accurate
i2c-pca-isa         & 0.078   & 0.250     & 42.1  & 53012\% & 75.25\%/112.24\%    \\\hline % not accurate
mv643xx \_eth.c     & 0.183   & 0.498     & 102.2 & 6443\%  & 1.23\%/7.54\%   \\\hline % not accurate
\end{tabular}%}
\label{tableRes}
\end{table}%

As we can see from the results, although lots of warnings are reported
by static analysis, these warnings can be reduced by symbolic execution or simulation.
In our experiment, most false positives are caused by unknown access type in external
functions or conflict path constraints. For example, if an ISR call an external function and a
SV is its argument, we regard this type of access as write since
static method may not know whether it's read or write.
The other reason of false positives is the priority,
programs without explicit interrupt lines will introduce more false positives.
We skip symbolic execution if the target driver does not require
external input. Note that some drivers require specific devices,
Simics could simulate most characteristics of these devices so that these drivers could be tested.
After static analysis, symbolic execution and dynamic simulation,
the validated data races are all real races except that the second
program has false negatives (discussed in section \ref{sec:dis}).

\commentty{The table needs to include more information:
the number of races explored by symbolic execution,
the inputs generated by symbolic execution, the iterations of
symbolic execution. It is also good to show the
amount of time taken in each step. Are interrupts have different
priorities? How priorities affect race detection effectiveness
(with and without considering priorities)? How did you inject
races?}

\wy{I only add a column for the table. And introduce priority of ISR and how to inject races}

\commentty{There are no results on bug fixing.
I suggest the follows: 1.
whether the patch is verified by developers or not.
If the patch cannot be verified (e.g., by fault injection),
whether it passes test cases. 2. the performance overhead
of the patch, comparing to manual fix. See the CFix paper.
}

\wy{I haven't test the performance overhead... Following is the result of automatic repair.}

We instrument interrupt enable and disable operations to verify the effectiveness
of automatic repair. After automatic race repair,
none of validated data races occur even we forcible trigger corresponding interrupts by simulation.

We implemented two ways to simulate embedded programs: ``out-of-tree''
build and ``in-tree'' build. ``out-of-tree'' build means that the source
for the kernel module is somewhere in our home directory structure,
not the kernel source directory like the standard device drivers that
come with Linux. The other difference between ``out-of-tree'' build
and ``in-tree'' build is that ``in-tree'' build requires less
human intervention, but we need to compile the kernel rather
than just compile kernel module.

According to the experiments, we can draw the following results:

1. For the subjects used in the experiment (small interrupt drivers),
our static analysis can effectively detects almost all data races.
Moreover, our approach is able to handle nested interrupts with
different priorities, rather than only deal with data race between
tasks and interrupt handlers. However, when the code structure
is complex (structures, arrays), it is difficult to ensure satisfied
accuracy, which may result in many false positives.

2. Dynamic simulation can identify most false positives.
Execution paths are provided to explain where and how does a
data race happen. In addition, our approach can provide priority
for each races, reducing the cost of manual validation.
Currently, some work should be done manually.
Compared to ``in-tree'' build, ``out-of-tree'' build runs in
a different environment, the other main difference is
that ``in-tree'' build is more difficult to instrument,
which leads to three drawbacks of build-in kernel mode,
can not rolled back, unable to control execution path and
can not ensure the path is indicated by PDR. However, ``in-tree'' build
can ensure less human intervention and higher efficiency.

3. Static analysis and dynamic simulation can be supplementary to
each other. For example, we do not make any instrumentation when
using ``in-tree'' build. Therefore, we can not ensure the execution
path is expected. However, if static analysis indicates that shared
resources only access once in tasks and interrupt handlers.
We can ensure the execution path is the same as the path
indicated by static analysis.

\subsection{Discussion}
\label{sec:dis}
\textbf{Limitation:} In experiment, we find some limitations of our approach:

1. Our approach can only deal with data races belong to order
violation. Data race caused by atomicity violation is not well handled.
As we mentioned above, our approach only considers write access to SV in ISR.
After experiment, we found that data race caused by automatic violation is
unconsidered. Codes in Listing \ref{falsenage} shows a example.
If the execution is preempted by function \textit{isr} right
before line \ref{falsenag:cri}, then variable \emph{StepsTemp}
in the ISR is not as expected since variable \texttt{DistanceSteps}
at line \ref{falsenag:err} should be {\tt 0} instead of {\tt 0xffff}.

\begin{lstlisting}[float=tp , language={[ANSI]C}, caption=False negative in dynamic validation, label=falsenage,  basicstyle=\ttfamily\footnotesize, numbers=left]
void put()
{
  if(DistanceSteps == 0xffff)
    DistanceSteps=0; (*@\label{falsenag:cri}@*)
}
void isr()
{
  StepsTemp=MAXSTEP-DistanceSteps; (*@\label{falsenag:err}@*)
}
\end{lstlisting}

2. Some functions are so simple that are optimized as inline function
by compilers. In this case, breakpoint for these functions will not be triggered.
In order to avoid this, we need to disable optimization for these functions.

3. Many false positives in static phrase are caused by nested interrupts,
because we can't determine the priorities of the two interrupts if
their priorities are all dynamic assigned. These false positives result in more validation
time in symbolic execution and dynamic simulation.


==> Sections/Introduction.tex <==
% !TeX root = ../bare_conf.tex

\section{Introduction}

Modern embedded systems are highly concurrent, memory, and sensor intensive, and run in resource
constrained environments. They are often programmed using interrupts to provide
concurrency and allow communication with peripheral devices. Typically, a peripheral
device initiates a communication by issuing an interrupt that is then serviced by an
interrupt service routine (ISR), which is a procedure that is invoked when a
particular type of interrupt is issued.  The frequent use of interrupts
can cause concurrency faults such as data races to occur due to interactions
between application tasks and  ISRs.  Such faults are often difficult to detect,
isolate, and correct because they are sensitive to execution interleavings;
therefore, they often occur intermittently and unpredictably.
For example, a number of people received fatal radiation overdoses
in the Therac-25 incidents~\cite{X}. This failure was due to a race
condition in which a keyboard interrupt handler participated.
The race could be triggered only by a particularly fast typist.

A common practice when testing for
concurrency faults is to execute many runs of a program
in the hope of exercising interleavings that cause
races.  This approach is known as \emph{stress
testing}~\cite{Park09}.  However,
existing approaches for randomly forcing interrupts is inefficient and
non-reproducible~\cite{Musuvathi08}.
In the ideal case in which randomly invoking interrupts does
expose faults, it may miss faults that can occur due to other interleavings.
%Further, a recent
%study has shown that the likelihood of executing the
%same interleaving patterns during each run of stress
%testing is high~\cite{Park09}, limiting the approach's
%effectiveness at exploring unexercised interleavings.

Many techniques have been proposed to improve stress
testing at the thread level by developing
algorithms and techniques to detect address data races,
including static analysis~\cite{Praun2003,Flanagan2003,Williams2005b,Naik2009,Joshi2012},
dynamic monitoring~\cite{Kahlon09,Marino2009,Bond2010,Effinger-Dean2012},
schedule exploration~\cite{Visser2003,Sen2007,Musuvathi2008,Sen2008,Coons2010,Burckhardt2010a},
test generation~\cite{pldi2012,icse2012-ballerina},
and concurrency fault repair~\cite{X}.
These techniques, however, focus on thread-level
races rather than process-level races.
Applying these directly to interrupt-driven software
is not straightforward.
%
First, interrupt-driven programs employ a different
concurrency model. The implicit dependencies between asynchronous
concurrency events and their priorities
complicate the happens-before relations that are used for detecting data races.


Second, controlling interrupts requires fine-grained execution control; that is,
it must be possible to control execution at the machine code level
and not at the program statement level, which is the granularity at which many existing techniques operate.
Third, occurrences of interrupts are highly dependent on hardware states;
that is, interrupts can occur only when hardware components are in certain states.
Existing techniques are often not cognizant of hardware states.
Fourth, interrupt-driven embedded systems typically have timing constraints.
Fixing data races in these systems is beyond simply enforcing synchronization
operations, but must ensure that their timing constraints are not violated.

%There are several techniques for testing embedded
%systems with a particular focus on interrupt-level
%concurrency faults~\cite{AST10Higashi, Regehr05, lai08nov}.
%For example,  Higashi et al.~\cite{AST10Higashi} improve
%random testing via a mechanism that causes
%interrupts to occur at all instruction points to
%detect interrupt related data races.
%However, these techniques rely on existing test inputs and could miss races
%that could otherwise be detected by other inputs. In addition, these techniques
%do not account for the implicit dependencies among tasks and interrupts due to
%priorities. Furthermore, none of existing techniques can automatically fix data
% races.



%By analyzing a large number of troubleshooting cases, we divide dynamic timing errors in interrupt-driven programs into the following four categories: 1. Data race. Data Race \cite{kahlon2007fast, abdelqawy2012survey, raza2006review, hafeez2012techniques, yu2005racetrack} is one of the most common concurrency bugs. In general, a data race occurs when multiple threads access the shared variables concurrently without appropriate synchronization, and at least one of them is write. 2. The time-out problem. During system running, some uncertainty leads to time-out of interrupt, tasks or subroutines and thus result in a system error. 3. Shared identity issues. The system associates interrupt, tasks and subroutines with each other by a shared identity. If the shared identity is inconsistent during program execution, it will lead to a system error. 4. Data integrity issues. It happens when a shared variable with multi-byte is preempted by an interrupt when the variable is accessed.

%Among the above type of problems, data race is one of the most frequent problems. The main reasons are as following: 1. To achieve data communication, there are a large number of shared resources in embedded systems. Interaction particle size between main task and interrupt handler is hard to design and implement, resulting in frequent data race. 2. Generally, the purpose of interrupt handler is to interact with data, which leads to frequent access to shared resources. 3. In some cases, some shared resources are not specifically protected because of the high real-time requirements. But this optimistic design will often be broken by the iterative update of software version and the inconsistent of program design and implementations, which will eventually lead to the occurrence of data race.

%Data race is also one of the most difficult problems. Therefore, how to effectively detect data races as early as possible is an eager prominent problem for both industry and academia. Existing data race detection approaches mainly include two categories: static analysis and dynamic testing. The static program analysis approach scans software source code to discover the code segments that possibly happen in parallel, and reports warnings for possible race conditions. Each warning needs to be manually inspected to check whether it is indeed a true data race. The key advantage of the method is that data races can be discovered and fixed before software integration and deployment. The key limitation is that the reported data races warnings contain too many false positives which mainly due to the lack of software execution information, thus each false positive wastes a huge amount of human effort on manual source code inspection. The dynamic testing approach instruments special code into software so that data race occurrences can be detected during in-house execution, and properly processed such as terminating software execution or tolerating the bugs. The key advantage of the method is that they rarely have false positives because they have software execution information. The key limitation of it is that they incur an excessive amount of performance overhead and the quality of testing depends on how many pathes it can execute. Therefore, false negatives may exist since we cannot perform exhaustive testing. Interrupt-driven programs are platform dependent. Testing could not detect data races when the test environment is different from the expected platform. Testers always face a dilemma. On the one hand, it is difficult to identify data races without testing the real interrupt-driven embedded system since race condition only occurs at specific scenario. On the other hand, even we found data race by testing real equipment, it is too late since the interrupt-driven program has already been integrated into the hardware and the cost of fix data races is expensive.


This paper presents \Name{}, an automated tool that combines static analysis,
symbolic execution and dynamic simulation to detect, validate and fix data races
in interrupt-driven embedded systems.
\Name{} first employs static analysis to identify code locations for potential
data races. In the second step, \Name{} uses symbolic execution
to generate data input and interrupt interleavings to validate potential
races and eliminate false positives. \Name{} leverages
the virtual platform's abilities to interrupt execution without affecting the
states of the virtualized system and to manipulate memory
and buses directly to force interrupts to occur.
Finally, \Name{} applies fix strategies by inserting interrupt
disable and enable operations at the hardware level to prevent
faulty interleaving, with a best effort to avoid deadlocks and excessive
performance losses.

To evaluate the effectiveness of \Name{}, we apply the approach to
\wym{??} embedded system benchmarks with both known and
previously unknown data races.
Our results show that \Name{} precisely
detected data races and successfully
fixes data races without causing deadlocks or
excessive performance degradation.
To the best of our knowledge, none of these race can be reproduced
automatically using existing techniques.
Furthermore, the time taken by \Name{} to detect, validate
and fix races is typically a few minutes,
indicating that it is efficient enough for practical use.

In summary, this paper contributes the following: \begin{compactitem}
  \item An automated framework that detects, validates and fixes
  data races for interrupt-driven embedded systems.

  \item The first approach to synthesize data inputs and interrupt interleaving
  schedules to validate data races.

  \item A practical implementation and empirical evidence that the approach
    effectively detects and fixes data races in real-world interrupt-driven
    embedded systems.

\end{compactitem}

The rest of this paper is organized as follows. Section \ref{sec:background}
introduces backgrounds, and Section \ref{sec:mod} introduces our method.
Section \ref{sec:imp} describes our evaluation of our method, and
Section \ref{sec:ret} provides details on related work.
Finally, Section \ref{sec:clu} concludes the paper. 

==> Sections/Method.tex <==
% !TeX root = ../bare_conf.tex

\begin{figure}[!t]
\centering
\includegraphics[scale=0.5]{Figures/arc}
\vspace{1ex}
\caption{\small The overview of our \Name{} framework.}
\vspace*{-15pt}
\label{fig_sim}
\end{figure}

\section{\Name{} Approach}
\label{sec:mod}

We introduce \Name{} whose architecture is shown in
Figure~\ref{fig_sim}.
The rectangular boxes contain the
major components: a \textit{static analyzer}, a
\textit{test case generator}, and a \textit{race healer}.
\Name{} first employs static analysis (SA)
to identify sources of race conditions.
Next, \Name{} invokes symbolic execution to generate
test inputs and interrupt schedules that can reach
the potential racing sources. \Name{} utilizes
the virtual platforms to exercise the inputs and
force the interrupts to occur at specific program
locations specified in the interrupt schedule.
The output of this step is a set of real racing pairs.
Last, the race healer generates patches to fix races
by enforcing interrupt disabling and enabling synchronizations.
It first determines where to enforce the synchronizations
and then generates patches using static code transformation.
The race healer employs several heuristics to find the best
patches considering correctness, performance, and patch simplicity.

\subsection{Static Analysis}

In the static analysis phase, \Name{} identifies
code locations of potential races for guiding
test case generation and race validation.
It first identifies shared resources and interrupt
synchronization operations. It then constructs
an event constraint model that describes the partial
order relations of the concurrency events in tasks
and interrupt handlers. Finally,
the static analyzer performs context-sensitive analysis to
identify a list of potential racing pairs.
The racing pairs are used for
guiding test input generation and dynamic validation.

\subsubsection{Shared Resource Identification}

Race conditions are generally caused by inappropriate synchronized
access to shared resources. So precisely detecting shared
resources is key to race detection.
In addition to shared memory that are considered by thread-level
race detection techniques,
\Name{} also accounts for hardware
components that are accessible by applications and device drivers,
including device ports and registers.
\commentty{How and/or what algorithms do you use to identify shared
resources?}

In practice, we identify shared resources by the pattern of  them. Namely, memory or registers used by two or more tasks are regarded as shared resources. The pattern includes two types, inter-procedure, intra-procedure shared resources. Therefore, we construct inter-procedure Control Flow Graph (CFG) to help us identify shared resources.
After identify shared resources.
Each detected shared resource is represented by a
5-tuple ``$<M, L, AV, V, T>$''. \emph{M} represents its function name;
\emph{L} represents the position where shared resource is accessed;
\emph{AV} represents resource's name in the function; \emph{AV}
can either be an alias or a real name (real name is the name when
the resource is declared); \emph{V} represents real name of this
resource; \emph{T} represents access type, read (represented by R)
and write (represented by W). The result of this phrase is a list of
the 5-tuple named as resources list (RSL).

%We detect shared resources according Algorithm \ref{alg:idenSRs}.
%The basic idea of identifying shared resources is to identify resources
% accessed by both tasks and ISRs.
%For each function, we record resources the function accessed (lines
% \ref{isr:id} and \ref{isr:str}).
%When all functions are analyzed, we extract and record shared resources based
% on accessed resources (line \ref{isr:ext} and \ref{isr:rec}).
%Every detected shared resource is represented by a
%5-tuple ``$<M, L, AV, V, T>$''. \emph{M} represents its function name;
%\emph{L} represents the position where shared resource is accessed;
%\emph{AV} represents resource's name in the function; \emph{AV}
%can either be an alias or a real name (real name is the name when
%the resource is declared); \emph{V} represents real name of this
%resource; \emph{T} represents access type, read (represented by R)
%and write (represented by W). The result of this phrase is a list of
%the 5-tuple named as resources list (RSL).

%\begin{algorithm}
%\caption{Identify shared resources}
%\label{alg:idenSRs}
%\begin{algorithmic}[1]
%\raggedright
%\REQUIRE Programs
%\ENSURE SharedResources
%\FOR{function in Programs}
%  \STATE res = identifyAccessedResources(function);\label{isr:id}
%  \STATE storeAccessedResources(res);\label{isr:str}
%\ENDFOR
%\STATE SRs = extractSharedResources(res);\label{isr:ext}
%\STATE recordSharedResources(SRs);\label{isr:rec}
%\end{algorithmic}
%\end{algorithm}

\subsubsection{Synchronization Identification}

The interrupt synchronization operations
typically involve interrupt disabling and enabling operations.
By default, \Name{} records standard Linux interrupt APIs,
including {\tt disable\_irq(int irq)}, {\tt disable\_irq\_nosync(int irq)}
and {\tt enable\_irq(int irq)}, where the {\tt irq} parameter
indicates the interrupt vector number (i.e., the unique
ID of an interrupt).
One challenge is the implicit interrupt operations in which
an interrupt is disabled or enabled by directly manipulating
hardware bits. \Name{} performs a conservative analysis by
putting all hardware operations into a list. In the dynamic analysis
phase, \Name{} monitors the hardware states to determine
which hardware operations are related to interrupts.
%
%Main purpose of interrupt resource detection is to detect
%interrupt enable or disable operations. So that interrupt
%enable status for shared resources can be calculated in
%control flow and data flow analysis. In most embedded systems,
%coding is rather flexible. Interrupt vector's initialization and
%interrupt switch would be various in different systems,
%platforms and processors. For example, Linux interrupt
%mechanism employs Interrupt Descriptor Table (IDT) \cite{corbet2005linux}.
%IDT includes 256 interrupt descriptors which are associated by
%interrupt or exception respectively.
%Interrupt switches in Linux depend on three functions:
%disable\_irq(int irq), disable\_irq\_nosync(int irq) and
%enable\_irq(int irq).
Interrupt APIs can vary across different kernels
and architectures. In this case,
a configuration file is provided, that allows users to
specify the names of APIs.
The output of the step of synchronization identification
is a 4-tuple $<M, L, I, T>$, where \emph{M}
represents function name; \emph{L} represents the position
where interrupt enable operation is called; \emph{I} represents
the interrupt vector number; \emph{T} represents the type of
interrupt operation (i.e., enable or disable).


\subsubsection{Potential Racing Source Identification}

In this step, we identify shared resource pairs
that may race with each other from all shared resources.
These pairs are used for guiding symbolic execution
to generate test inputs.
%We construct an interrupt-enabled
%inter-procedure control flow graph (IICFG) that describes
%data and control flow of variables across application tasks
%and interrupt handlers.
%\commentty{Better to have a graph.}
We first build a control flow graph (CFG) for each
task and interrupt handler. For each shared variable
in the CFG, we maintain a map that record
the current interrupt status (i.e., enable or disable)
and priority (in the case of dynamic priority adjustation).
For example, \commentty{add an example} \wy{added} if interrupt line 9 is disabled,
the corresponding field in the map is set to 1, denotes that interrupts with 9th
interrupt line will not be checked for data race until the interrupt line is re-enabled.
For each shared resource $SV$, if there exists another shared
resource $SV'$ in a higher priority interrupt and
that interrupt is disabled at $SV$, ($SV$ and $SV'$)
is a potential racing pair.

\commentty{I move the path computating down to
the symbolic execution section.}
%\wy{add the output of static analysis.}
%Our static analysis provide outputs for further usage.
%The first one is potential race warnings for dynamic simulation,
%automatic fix or manual verification.
%The second one is paths for each potential race warnings.
%We provide paths from the beginning of the program to the race points.
%These paths are used for symbolic execution so that symbolic
%execution could collect path constraint along the paths.


\ignore{
A CFG is a representation, using graph notation,
of all paths that might be traversed through a program during its execution.
Each node in the graph represents a basic block.
In data race detection, since races occur when accessing
shared resources which are distributed in a part of all branches,
most statements in blocks are useless at static analysis phrase
for data race detection. Therefore, we eliminate CFG according to
whether a path contains statements accessing shared resources,
enable or disable interrupts and branches.
This CFG is more concise than traditional CFG and we name
it as Reduced Control Flow Graph (RCFG). To generate RCFG,
we need resources list, interrupt resource list (ITRL) and
each function's CFG. For each CFG's basic block \emph{B},
if some statements access shared resources or interrupt
enable operations according to SRL and ITRL.
We keep these statements. Note that branches in source
code will affect CFG's logical. So if a statement belongs
to if, while, for, goto statement, function call and so on,
we will also keep these statements.
Finally, we add the constructed RCFG to a set named RCFGs.

\textbf{IIRCFG construction:}
Most of time, trigger of interrupt is uncertain in
interrupt-driven programs. The uncertainty is the
primary reason for data race. However, interrupt
will not always result in data race, but when the
interrupted task and Interrupt Service Routine (ISR)
access the same shared resource and ISR writes shared
resource will result in data race. Interrupt Inner
Reduced Control Flow Graph (IIRCFG) is focus on these
moments. This section introduces how to generate IIRCFG
from RCFG, SRL and ITRL. We interconnect all of the tasks
(which means ISRs are not included) between the call connections,
which constructed a global RCFG. For every task in CFG, add it to
the global RCFG if it is not in it. Then find if there is a call
in the task, if there is, point the caller to the callee.

Then we try to find appropriate interrupt trigger time.
Interrupts will be inserted to the global RCFG to construct
IIRCFG. Bit vector \emph{INTB} is used to record current
interrupt enable status. We traverse the global RCFG by
depth-first search to examine every statement of RCFG
interrupt switches, and to update the bit vector \emph{INTB}.
While checking the statement of shared resources (SRs) accessed,
if there exists a higher priority interrupt can also write to
the shared resources. It constitutes a potential data race.
We insert the begin node and end node of the interrupt
into the statement to constructed potential data race.

Noted that similar to the situation that tasks could be
preempted by ISRs, ISR with low-priority also can be
preempted by a higher priority ISR, which will lead
to a data race caused by nested interrupts.
Therefore, we traverse RCFG tasks as well as
all the other interrupt handlers' RCFG.

\textbf{IIRCFG serialization:}
IRCFG includes a list of potential data race
where may occur while program is executing.
However, in order to facilitate race validation
and repair, we need to make the CFG serialization
to extract each potential data race's execution sequences.
The serialization process is done by graph traversal algorithm,
the result of serialization is two lists: shared resources
access list (SRAL) including each SR access point and
shared resources sequences list (SRQL) storing execution
sequences corresponding to each access point in SRAL.

In SRAL, each access point is a 6-tuple ``$<M, L, P, AV, V, T>$''.
Where, \emph{M} and \emph{L}, respectively, is the function name
and line number of the access. \emph{P} represents the priority
of the task (the lower the number is, the higher the priority is.
nine denotes a task). \emph{AV} is an alias for the shared
resource in the function, and \emph{V} is the real name of the
shared resource, \emph{T} represents the type of access operations,
which can be divided into read (W) and write (R) two types.

In SRQL, each record is a series of executions, indicating
possible execution sequences corresponding to the shared resource.
Each record consists of a number of execution units formed ``$M <X>$'',
where M represents the name of the function. When the statement is a
branch statement, \emph{$L | Z$} is used to represent a branch,
where \emph{L} refers to the line number and \emph{Z} means that
the branch is true or false; \emph{L} represents a line number
when the statement is a non-branch statement.

It's worth noting that the main purpose of the two list is to locate
the position of data race, not only could it help developers fix data
races, but also it's helpful in dynamic validation and automatic fix.

\textbf{Potential data race analyses:} Based on SRAL and corresponding
SRQL, we can predict potential data race according to a principle,
and give potential execution sequences of the potential data race.
The principle is that when different priority functions (common tasks
and interrupt handlers, low-priority interrupt handler and the high-priority
interrupt handler) simultaneously access the same shared resource, and
high-priority interrupt handler writes the shared resource, the data will
have the potential to race. Output of static analysis is named as potential
data races (PDRs) or static warnings. Static analysis can report different
shared resources such as shared variables, shared port, registers,
and so on. However, more complicated data race conditions like race
with dependency (Interrupt enable operation could be disturbed by
other tasks or interrupt handlers) will not be considered as it
cannot be simulated in next stage.

Note that the interrupt handler accessing to shared resources
must be a write operation rather than multi-threaded scenarios'
commonly defined: ``at least one of the accesses is for writing''.
For example, example in Listing \ref{exp2} demonstrates it.
If \emph{interrupt1} is triggered when \emph{task1} is writing
shared variable data (line 6), since the shared variable data in
\emph{interrupt1} performs read operation (line 17), meet the
definition that at least one of accesses is write. However,
this doesn't cause data race. The reason is that the interrupt
itself is atomicity. All operations performed to shared variable
data by \emph{interrupt1} is consistency, which makes the read
operation performed by itself will not be out of data, unless
there is a higher priority interrupt handler, we might call
it \emph{interrupt2}, preempts it and changes the value of the
shared variable, but it belongs to the race between \emph{interrupt1}
and \emph{interrupt2}. As we can see, traditional race definition in
multi-threads program does not meet the requirement. This race is
actually not so harmful that we will not put it in the report
as potential race. %For the example named \emph{keyboard Driver} in Listing \ref{exp3}, its result provided by static analysis is show as Figure 2, as we can see, lots of warnings are reported.

In order to avoid false negatives, we designed a static analysis
that detects races as many as possible. It may report some false
positives. Moreover, not all the races will cause harm to the
system (some races are dangerous, it will cause the program to
crash or behave in unusual ways. But some will not affect the
behavior of the program, such as a contaminated data is always
immediately reset to the normal value).

Therefore, such a conservative strategy in static detection
will affect its applicability, resulting in false positives.
However, if we perform a dynamic validation after the static
analysis, it has some advantages: Firstly, the static analysis
introduces a few false positives and avoids false negatives.
Dynamic validation would get rid of as many false positives as
possible. It will ensure the accurate and comprehensive for final
detection results. Second, although not all the races are harmful,
finding harmless races in the program will also help developers to
distinguish and confirm whether the practice is intentional or
 potentially dangerous (such as accidentally introduced by project
 iteration, and it may become harmful race issues in the next iteration).
 }

\subsection{Guided Symbolic Execution}

We propose a new symbolic execution procedure to compute
test inputs in an interrupt-driven program.
This step differs from prior works on diagnosing concurrency
bugs using symbolic execution~\cite{Marinescu12,Farzan13} in that all
these prior works focus on multi-threaded programs.
In contrast, interrupts and tasks have asymmetrical preemption relations.
First, all interrupts can preempt non-interrupt code, whereas non-interrupt
code can never preempt any interrupt. Second, interrupts are often scheduled
using fixed priorities, resulting in asymmetrical preemption relations
among interrupt handlers.
Internally, we leverage the KLEE symbolic virtual machine~\cite{Cadar08} to
implement the goal-directed exploration of the program to traverse the program
locations involving potential races.

Give the racing pairs computed from the static analyzer, \Name{}
performs a depth-first traversal on the inter-procedural
control flow graph (ICFG) of PuT to compute a set of simple paths
that contain shared resources. These paths are used to guide
symbolic execution for generating inputs.

%Execution paths in interrupt-driven programs usually depend on lots
%of external inputs like registers, parameters, data buffers and so
%on \cite{yu2016vdtest}. Dynamic validation only with the potential
%race pair may result in low efficiency because the program may
%not execute the race path. Therefore, a test case that guides
%the program to execute the path indicated by potential race
%pair should be calculated to improve the efficiency.

%%%%%%%%%Need revision. The logic is not clear.
%Although many symbolic execution techniques have been are proposed in
%recent years, most of them . Note
%that scenarios in interrupt-driven program is different from
%scenarios in multi-thread programs. In multi-thread program,
%two threads may execute alternately.

\wy{Illustrate different constraints we required.}
The key part in symbolic execution is to traverse
the program path to collect path conditions (PCs).
A test input is generated by
solving path conditions using an SMT solver.
Since calling an interrupt handler may change the control
flow of current running task or interrupt handler,
we serialize the interleaving of the task and the ISR
that contain potential racing events.
In other words, in symbolic execution,
the first part of path constraints are collected along tasks,
when symbolic execution reaches the interrupt trigger point,
it begin to collect the last part of the path
constraints which  is in the ISR.
Besides the path constraints, other constraints should be provided so that symbolic execution
could generate effectiveness test cases. These constraints for data race in interrupt-driven programs includes failure constraints,
read-write constraints, synchronization constraints, interrupt enable constraints and memory constraints.
The combination of these constraints indicates data races.
Read-write constraints, synchronization constraints and interrupt enable constraints are solved in static phrase, which means that static warning are all meet these constraints.
Memory constraints are memory access orders, we use SC order.
Therefore, symbolic execution is focus on path constraints. 

In embedded systems, inputs involve hardware data
buffers and registers.
In order to force symbolic execution
engine take these inputs into consideration, we explicitly
point out data buffers and registers should be symbolized.
Some symbolic execution engines like KLEE \cite{KLEE}
provides an API named as \emph{klee\_make\_symbolic} to mark a variable as symbolic.
%
%Symbolic execution engine could begin to analyze interrupt-driven
%program after ISR serialization and input symbolization.
%However, path explosion will become the main problem and lots
%of path solved by symbolic execution engine is useless since
%
To mitigate path explosion,
we only consider the pathes indicated by static analysis.
Therefore, we implement a guided symbolic execution that only
gather constraints related to the target paths.
%If we encounter loops and a shared variable is in the loop, we
%only gather constraints for the loop. If some iteration could
%reach the shared variable, we merge the constraints in the loop
%with original constraints collected before the loop. If shared
%variable is outside the loop, we only iterate the loop once and
%continue to explore the following paths.
%
%Although symbolic execution works on paths in this phrase,
%it solves other race constraints implicitly.
%As far as we know, a data race consists of the following
%constraints \cite{machado2015concurrency}: path constraints,
%failure constraint, read-write constraints, synchronization
%constraint and memory constraints. Read-write constraints and
%synchronization are implicitly solved in static phrase,
%which means that static warning are all meet these constraints.
%So we need to use symbolic execution to solve path constraints.
%Memory constraints is memory access order, although we don't
%mention it, we use SC order.

The way how we enumerate paths is that we obtain all possible
paths to shared variables by static analysis, then we guide
symbolic execution by these paths.
\commentty{How paths are selected? Do you randomly select
a path or employ heuristics? How do you determine loop
iterations?}\wy{Added explainations}
Most symbolic execution engines collect and solve path constraints
based on depth-first search, breadth-first search or random search.
Therefore, it may takes long time for them to collect the path constraints pointed by static analysis.
In order to accelerate symbolic execution, we rewrite the path exploration strategy so that
symbolic execution engine only explore paths indicated by static analysis and skip unrelated paths.
In other words, we prune paths that are not given by static analysis to improve the efficiency of symbolic execution.
Note that two or more paths could reach the race points, the way to collect path constraints in these paths is depend on
search algorithm. If the first path constraints can not be solved,
symbolic execution engine will try the next paths until all paths are explored.
If we encounter loops and a shared variable is in the loop, we gather constraints for the loop
and add these constraint to a empty constraint set.
\commentty{What does ``only gather constraints for the loop'' mean?}
\wy{change the description}
If we could reach the shared variable within a limited iterations, we merge the constraints in the loop with original
constraints collected before the loop. Otherwise we report the situation as time out. If shared variable is outside the loop,
we only iterate the loop once and continue to explore the following paths.

For each static
warning, three possible results may generated by symbolic execution.
The first output is a list of test cases, which means the path is able to reach.
The next result is a unreachable warning or message, which denotes that
the static warning is a false positive. The last output is a message
indicating the unsolvable constraints. The reason may be execution
time-out, limitation of constraint solver or unknown external functions.
\commentty{For the above sentence, how do you determine these are
the cases? by just looking at the KLEE output messages?}
\wy{Yes, symbolic execution engine provide these information.}
After the symbolic execution, we continue validate static warnings except
for the second result.
\commentty{If a time-out occurs, no test inputs would be generated.
Then how do you validate the races that must be exercised by
certain inputs?}
\wy{Race warnings who are simulation time-out will be forcible controlled
to reach the paths. These races will be reported with lower priorities}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%   2016.7.13: add a moti-example for the whole artical.


\subsection{Schedule Generation and Replay}
\label{sec:DYN}

After symbolic execution, we then perform dynamic simulation to validate
the static warning. As we mentioned above, we serialize programs to compatible
with symbolic execution engine. The reason we serialize the task and ISR is
that simulation technique could directly invoke the corresponding ISR at most
required program execution point. With the help of this technique, interleaving
of a task and a ISR could be regarded as executing sequentially. Moreover,
simulation technique could directly assign data buffers or registers with
the data pointed by generated test cases, which could improve the
performance of simulation phrase.

\commentty{This section needs to be re-written. There
are too many implementation details. We need to show
algorithmatic novelty. I think we can add a new theory
on happens-before/partial order relations that specific
to interrupt-driven programs.}

\wy{This section is based on SimTester, we improve it so that
dynamic simulation is able to identify two or more races for one shared variable in one function.
for example, f(){sv=1;sv=2;} isr(){sv=3;}

I'm not sure how to add the theory, how can we use the theory to control the simulation?}

\wy{TODO: Here}

\ignore{
\subsubsection{Validating warnings via Automatic Simulation}
Static analysis provides a good foundation for data race detection.
However, it is a static analysis modeling process and false positives
due to accuracy problem are inevitable. The cost of manual validation
is far more expensive than expected. However, run-time validation also
face a problem that data race depends on the specific execution sequence
and the advent of interrupt on the system is uncontrollable, which makes
automatic validation even harder.

Testing interrupt-driven program may heavily rely on hardware and
interrupt scenario. Due to the nondeterministic trigger time of
interrupt, it is harder to reproduce the race scenario.
In this paper, we apply simulators, such as Simics, to provide
a virtual execution platform as well as user controlled execution scenario.
In order to reproduce race scenario, simulator will trigger expected interrupt
when program accessing a variable indicated by static warning.
Thus, the implementation of dynamic simulation can effectively
reduce false positives.

\begin{figure}[!t]
\centering
\includegraphics[width=2.5in]{Figures/dynProc}
\caption{Procedure of dynamic simulation.}
\label{fig:dynproc}
\end{figure}

\subsubsection{Dynamic simulation}
Dynamic simulation is divided into
three stages: breakpoint configuration, program simulation and
log analysis (Figure \ref{fig:dynproc}). At the first stage: each static
warning is analyzed so that we can set memory access breakpoints and execution
breakpoints. In order to obtain and analyze the memory information,
we also set the corresponding call back functions for these breakpoints.
At the second stage: we simulate the target program and
load the simulation scripts to validate static warnings. This stage records memory access
and function execution information. Finally, we analyze whether race occurred based on the log.

At the first stage, we config breakpoint based on Algorithm \ref{alg:confbrk}.
This algorithm takes a potential data race (PDR) and a boolean variable named \texttt{ifInsertMagic}
as input. The PDR is used to extract tasks, SR and ISRs so that we can set breakpoint for
them (lines \ref{conf:ana} to \ref{conf:ab}). \texttt{SRPos} is used to store the precise position of the SR.
The boolean variable is defined
to determine whether set MAGIC breakpoints or not. If it is set to true,
we first instrument MAGIC instructions and then set the breakpoint (lines \ref{conf:magbeg} to \ref{conf:ins}).
MAGIC breakpoint is a special type of breakpoint which could also call the
call back function when the breakpoint is reached. The instrumentation is used to locate the precise
position of shared resources. The reason why we instrument these instructions is that memory access breakpoint
can not distinguish two memory access in one function. For example, in Figure \ref{exp1},
lines \ref{exp1:cri} and \ref{exp1:read} both read the variable \texttt{packetsNumbe}.
If a read breakpoint for \texttt{packetsNumbe} is triggered, we are not able to distinguish whether
line \ref{exp1:cri} or line \ref{exp1:read} is executed based on the breakpoints we set. In contrast, if we
instrument a MAGIC instruction right before and after line \ref{exp1:read}. Then we can determine whether line \ref{exp1:read}
is accessed.

\begin{algorithm}
\caption{Config Breakpoint}
\label{alg:confbrk}
\begin{algorithmic}[1]
\raggedright
\REQUIRE PDR, ifInsertMagic
\STATE (tasks, SR, ISRs, SRPos) = separateFunctions(PDR);\label{conf:ana}
\FOR{f in tasks and ISRs}
  \STATE set execution breakpoint at entry point function addr of f;
  \STATE set execution breakpoint on function return instruction ret;
  \STATE set execution breakpoint on interrupt return instruction iretd;
\ENDFOR
\STATE set access breakpoint on SR;\label{conf:ab}
\IF {ifInsertMagic == true}
  \FOR{f in tasks and ISRs}\label{conf:magbeg}
    \IF {ifInsertMagic == true}
      \STATE instrumentMagicIns(SRPos);
    \ENDIF
  \ENDFOR
  \STATE set magic Breakpoint at magicBreakpoint;\label{conf:ins}
\ENDIF
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{Race Simulation}
\label{alg:racesim}
\begin{algorithmic}[1]
\raggedright
\REQUIRE PDR, C'
\ENSURE RL
\SWITCH{breakpoint}
  \CASE{function\_addr}
    \STATE  funclist.push(func\_addr, ebp, esp);
    \IF{funcaddr == ISR\_entry}
      \STATE log(``ISR entry''); \label{sim:isrent}
      \STATE isISR = true;
    \ENDIF
  \ENDCASE
  \CASE{ret}
    \IF{esp == funclist.top().esp}
      \IF{funclist.top().func == ISR\_entry}
        \STATE log(``ISR exit''); \label{sim:isrext}
        \STATE isISR == false;
      \ENDIF
      \STATE functionlist.pop();
    \ENDIF
  \ENDCASE
  \CASE{iretd}
    \IF{ebp == ebp\_switch}
      \STATE log(``iretd'');
      \STATE logNextProgramCount(); \label{sim:npc}
    \ENDIF
  \ENDCASE
  \CASE{SharedResource}
    \IF{ebp == funclist.top().ebp}
      \IF{isISR == false}
        \STATE log(``PuT'', SV, SVaccess, pc); \label{sim:put}
        \STATE ebp\_switch = ebp;
      \ELSE
        \IF{SVaccess == write}
          \STATE log(``ISR'', SV, SVaccess); \label{sim:sv}
        \ENDIF
      \ENDIF
    \ENDIF
  \ENDCASE
  \CASE{MagicIns}
    \IF{ifPathSatified()}
      \STATE  pathSatified = true;
      \STATE logExecutionInformation();
    \ENDIF
  \ENDCASE
\ENDSWITCH
\IF{isExecutionTimeOut()} \label{sim:timeb}
  \STATE changeExecutePath();
  \STATE getNextProgramCount();
\ENDIF \label{sim:timee}
\end{algorithmic}
\end{algorithm}

Algorithm \ref{alg:racesim} monitors
runtime states and controls execution paths. At the beginning,
all test cases run under the natural state execution.
If the tasks' execution sequence is the same as PDR's sequence,
simulator triggers the interrupt and check whether a race has
actually happened. Finally, simulator analyzes execution log
to determine whether races happened.
In the algorithm, races happen when the following conditions are satisfied. A shared variable is accessed at a task (line \ref{sim:put}),
then it preempted by an ISR (line \ref{sim:isrent}). The ISR should write the shared variable (line \ref{sim:sv}). When the IST finish executing,
the next instruction in the task to be executed is the instruction right after the SV access in task (line \ref{sim:npc}).
In some cases,
the execution sequence of a potential race does not satisfied.
Two reasons should be considered: first, the execution path
indicated by a PDR is not so easy to execute; second, this PDR
is a false positive. Therefore, we set a limited execution time
as time-out threshold.
At the beginning, the program is uncontrolled. When task's
execution time exceeds the threshold, Simics performs a
reverse execution to the nearest checkpoint and forces the program to run
the path indicated by the PDR. The nearest checkpoint is a execution point nearest to
the target paths, the execution point is collect during ordinary run.
When the simulator roll back to previous state, we skip branch conditions and directly set the program count to
the branch forward target paths (lines \ref{sim:timeb} to \ref{sim:timeb}).
In this way, it is possible to
ensure that all PDRs are dynamic validated. It will record
the priority of the PDRs named as RL for further usage.

\subsubsection{Output of dynamic simulation}

Output of dynamic
simulation is a validation for each PDR.
There are three results: first, the pdr is a data race
with the importance of the race. Second: program execution timeout,
the situation does not reach the shared resource in task.
If the execution path is forcibly controlled, two results may be
possible, the race is a false positive of static analysis;
or the task has not been executed. However, these two cases can
be distinguished by dynamic simulation. If the execution path
is not forcibly controlled, the data race can be either a false
positive or a real race. Third: this PDR is a false positive.
As far as we know, there is only one reason for this situation:
two interrupt handlers are the same function.

In dynamic simulation, lots of the steps needs to be done manually,
but these steps have the similar steps, such as selecting an
output of a static analysis, configuring dynamic simulation script,
and loading Simics and program under test (PuT).
These tasks can be done automatically by scripts. It not
only speeds up simulation process, but also greatly reduces
the manual work, increasing the efficiency of simulation and
enhancing the degree of automation.
}

\begin{algorithm}
\caption{Calculate Priority}
\label{alg:calpri}
\begin{algorithmic}[1]
\raggedright
\REQUIRE CFGs
\ENSURE priorities
\FOR{cfg in CFGs}
  \STATE weight = weight + controlled instruction / total instructions;
  \STATE funCount = funCount + 1;
\ENDFOR
\STATE weight = 1 - weight / funCount;
\end{algorithmic}
\end{algorithm}

\subsubsection{Race Ranking}

In software engineering, static warnings validation and
defects fix are both troublesome and labor intensive.
Particularly, if the static warnings include large numbers
of false positives, engineers must focus on meaningless work
that would seriously affect the progress of program development.
For interrupt-driven programs, validating false positives spends
more cost than ordinary projects.
\commentty{This is not true based on the experiment results.
There are not many false positives to validate.} \wy{But validate a false positive require more effort,
because we should consider lock state and irq enable state, instead of only lock state.}
As our approach forcibly
control execution paths, some races may not happen in production run.
Therefore, giving simulation results with priority can help
developers focus on harmful data races.

\commentty{I do not think I understand the whole logic
of prioritization. How do you rank these races? how do you
know one race is more important than another?}

\Name{} employs estimation algorithm to prioritize
racing pairs for validation.
The possibility of the races occurrence is the
consideration for the importance of the potential data races.
The more branches are controlled, the lower probability of the occurrence is.
Branch control means that we do not care about the condition of a branch any more, instead,
we directly force the program counter point to the instruction toward our paths.
If we do not control the program, then these races are reported with highest priority.
If we control branches, this means that we try to validate this warning as soon
as possible to avoid long validation time. Due to the reason that we do not know whether these skipped branches
are able to satisfy. Therefore, the priority ranking is based on the assumption that
each branch can be satisfied with the same possibility.
Note that the priority ranking is calculated in virtual platform, so we can know how many branches are controlled
by the virtual platform.
\commentty{Please justify the above sentence. Also,
how do you determine how many instructions
are controlled?}
\wy{explain the algorithm}
The algorithm is as Algorithm \ref{alg:calpri}, it averages each function's
controlled instructions divided by \emph{total instructions}.
Note that \emph{total instructions} are number of conditional instructions
from the first checkpoint to the race point.
\commentty{What is the first checkpoint? what is the target instruction?}
\wy{the first checkpoint is explained at algorithm `Config Breakpoint'}
Let us take keyboard Driver for example again. Assume we are validating
a PDR which is as follows:

$PDR(SRA2, SRA3) = \{task2<3 | T>, task2<4>\} R | \{irq\_handler1<15 | T>,
irq\_handler1<17 | T>, irq\_handler1<18>\} W.$

With test cases generated by symbolic execution, the output of our approach
verifying the code is listed at Listing \ref{text1}. Assume symbolic execution
fail to generate test cases, we could generate input by other ways like fuzzing.
However, Magic instrumentation mentioned above aims at these situation,
the modify source code is listed at Listing \ref{modKD}.
If the validation takes so long time that we have to chose a faster
way to validate static warnings, the simulator could forcibly control
the program to execute the target path. This step will downgrade the
priority of the path.

\ignore{

\begin{lstlisting}[float=t , language={[ANSI]C}, caption=Modified keyboard driver, label=modKD,  basicstyle=\ttfamily\footnotesize, numbers=left]
void task2()
{
  MAGIC(0);
  if(mode)
  {
    MAGIC(1);
    packetsNumber = packetsNumber - 1;
  }
  else
    bufferRemainCap++;
  MAGIC(2);
}
irqreturn_t irq_handler1()
{
  MAGIC(0);
  if(mode)
  {
    if(packetsNumber != -1)
    {
      MAGIC(1);
      packetsNumber = packetsNumber + 1;
    }
  }
  else
    ...
  MAGIC(2);
}
\end{lstlisting}


\begin{lstlisting}[float=t , language={[ANSI]C}, caption=Simulation result for instrumented program, label=text1,  basicstyle=\ttfamily\footnotesize, numbers=left]
irq_handler1 is added to breakpoint.
task2 is added to breakpoint.
SV:packetsNumber is added to breakpoint.
Successfully install callback function!
PuT: $packetsNumber$, Read, ffffffffa00ec097
Interrupt:10 is invoked
PuT: $packetsNumber$, Write, ffffffffa00ec097
ISR_entry
ISR_exit
Iretd
ffffffffa00ec097
RACE DETECTED
prio is:1.0000
\end{lstlisting}
}


\subsection{Automatic race fix}

For all validated race conditions, automatic data race fix will be performed
to heal data races. We design two repair strategies, the first one is
instrumenting interrupt disable and enable instructions, the other one is
mutual exclusion. The core idea of the first strategy is to instrument
interrupt disable and enable instructions (ie., disable\_irq(int irq) and
enable\_irq(int irq) in Linux) on tasks to avoid triggering the interrupt
which may result in data race. The PDRs' priority ranked in dynamic
validation is used to exclude races with lower priorities since these
races is forcedly controlled by virtual platform. Instrumenting interrupt
disable and enable instructions requires interrupt request lines which
are analyzed from static phrase. If the interrupt request line is dynamically
determined and it's local variable, we add a global variable to store the
interrupt request line. So that the we can know the interrupt request line
at any position. Note that we instrument interrupt switches on tasks instead
of ISRs. However, if the data race we try to fix is a data race caused by
two ISRs with different priorities, we should instrument interrupt switches
on the ISR with lower priority. If disable\_irq is called twice, the interrupt
line is not actually reenabled until the second call to enable\_irq \cite{corbet2005linux}.
Therefore, the fix strategy is flexible for two or more races in different tasks preempted
by the same interrupt. However, it's inefficient and a more efficient strategy should be provided.

%In contrast, repair data race by mutual exclusion is more efficient.
%We should instrument lock and unlock operations for critical sections
%in tasks and ISRs. In order to avoid introducing dead lock, all races
%are protected by the same lock.

The range of critical section is determined by the following algorithm:
Whenever a SV write in the main program is encountered, create a new
critical section until another write occurs. If no such a write occurs
at the end of the function, use the last read as the exit of the critical
section. In the cases of critical section overlapping, we need to merge
critical sections.

\commentty{I think only one strategy is needed. The pair of interrupt disabling
and enabling is actually a critical section. Some interesting points include:
determine the length of a critical section (e.g., when to enable an interrupt),
avoid deadlock, globle interrupt VS local interrupts. How to minimize the
performance overhead is important to embedded systems.
You also need to evaluate
your fixes interms of performance and deadlock.}


==> Sections/Relatedwork.tex <==
% !TeX root = ../bare_conf.tex

\section{Related work}
\label{sec:ret}
\subsection{Traditional data race detecting technique}
In the long term, a lot of work has been done to study the data race for concurrent programs. According to different techniques, they can be divided into the following methods. Lockset algorithm \cite{yu2005racetrack,savage1997eraser,o2003hybrid,pozniansky2003efficient}, but it can not be used at interrupt-driven system. Because lock is not the only way to prevent data race in interrupt-driven programs, and traditional lock set based detection does not take priority and preemption into consideration. Data flow and control flow analysis \cite{duesterwald1991concurrency, callahan1990analysis}, false positives are difficult to avoid by this technique. Happens-before relationship \cite{savage1997eraser, aspinall2007formalising, manson2005java}, limitation of the technique is that tracking happens-before relationship is often difficult. Model checking \cite{visser2003model, blanc2010race}, advantage of model checking is that it can be performed automatically, but it is difficult to abstract the program and build the model. Type system \cite{boyapati2001parameterized, flanagan2000type, agarwal2004type} is also an valued to detect data races.

\subsection{Date race tolerating}
Existing techniques that tolerate concurrency bugs includes always-on approach and failure-recovery approach. Always-on approach: this approach achieve data race tolerating by constraining program execution all the time. For example, Atomtracker \cite{muzahid2010atomtracker} and AtomAid \cite{lucia2008atom} group instructions into chunks and execute every chunk atomically. This approach constrains interleavings even during correct runs and relies on transactional memory or other custom hardware to achieve good performance. Failure-recovery approach: this approach \cite{veeraraghavan2011detecting, yu2009case} rolls back program execution to a recent checkpoint when errors occur, and prevents errors by re-execution.

AI \cite{zhang2014ai} presented a novel approach. The key observation behind this approach is that there exists a turning point \emph{t} during the manifestation of a concurrency bug: before \emph{t}, the manifestation is non-deterministic. After \emph{t}, the manifestation becomes deterministic. Thus if a concurrency bug can be anticipated before its turning point, its manifestation can be prevented by temporarily stalling a thread, which incurs little overhead. They find that the manifestations of most concurrency bugs involve an instruction \emph{I1} preceded by an unexpected instruction \emph{I2} from a different thread, where \emph{I1} and \emph{I2} access the same variable. In addition, postponing the execution of \emph{I2} can often prevent the bug (i.e., the execution of \emph{I2} is the turning point). Therefore, by calculating expected instruction for each SV in the test run, AI can tolerate concurrency bugs in production run. However, although AI can tolerate data race, it need more time to report the bug as this method waits data races to occur.

\subsection{Date race detecting methods for interrupt-driven system}
Data race has been a concern for long time and a lot of research is accumulated. Traditionally, we can divide detecting methods into static and dynamic testing.

\subsubsection{Static date race detecting}
Race in interrupt-driven program is generally believed that it is more complex and difficult due to the uncertainty of interrupt. HuoWei \cite{wei2011static} and Rui Chen \cite{chen2011static} proposed novel methods, but false positives remain a problem. Moreover, execution paths is not provided, which make verification work less effective. REGEHR et. Al. \cite{regehr2007interrupt} proposed an approach to transform interrupt-driven programs into multithreaded programs, and analyze these programs by multi-threads detection tools. However, although the data race caused by interrupt is similar to data race caused in multithreads, they are different in many aspects, which make it very difficult to equivalently transform programs. Therefore, this method is more difficult to avoid false positives.

\subsubsection{Dynamic date race detecting}
Regehr J et al. \cite{regehr2005random} attempted to use random testing methods for data race. When testing interrupts will be triggered according to a defined schedule. The performance of this method depends on the schedule. Higashi M et al. \cite{higashi2010effective} improved random testing, triggering interrupts when SVs are accessed and interrupts are triggered by instrumentation. This method is more effective but many instrumentations should be done manually. Even though our approach also need instrumentation, the instrumented positions can be automatically done by scripts.

Tingting Yu et al. \cite{yu2012simtester, yu2013simracer}, presented two simulation ways related with data races. SimTester \cite{yu2012simtester} uses Simics for detection. Data races can be detected base on system status monitored by Simics, This idea can be widely used as Simics can simulate different environments. However, it relies on test cases that cannot cover most execution paths. It will result in many false negatives. In contrast, our approach uses Simics to validate static warnings, which will consider more race scenarios than this method. SimRacer \cite{yu2013simracer} allows engineers to effectively test for process-level races by providing deterministic execution in multiprogramming systems. Its framework employs the Simics to observe system execution, to deterministically control occurrences of events, and to allow testing to target specific types of races. The framework allows engineers to focus only on applications under test without worrying about other events or applications in the system. Side effects from execution of applications not under test can be easily determined by querying current system states. By using Simics, its framework also operates at the binary level so it is capable of detecting races between applications written in different languages. It is also generalized, as it can be used on any system that can run on Simics.

\subsection{Data races repair}
As far as we know, there haven't been a automatic bug fixing tool that target at interrupt-driven programs. However, lots of automatic repair tools or techniques focus on concurrent problems in user space applications have been proposed.

AFix \cite{jin2011automated} is a system for fixing single-variable atomicity violations. It starts from an in house tool named CTrigger to dynamically detect atomicity violations. AFix then constructs patches for each bug. Once all patches are created, AFix tries to combine the patches to achieve better performance and code readability. Finally, thread noising techniques are used to test the fixes created by AFix.

ARC \cite{kelk2013automatically} is a framework for fixing data races and deadlocks in concurrent Java programs. It focuses on bugs detected by test cases. An analysis performed
by ConTest determines the classes and variables used concurrently. Note that a common problem for automatic bug repair techniques is the size of the search space of possible bug fixes. The search space of potential fixes is narrowed as ARC focuses only on those lines of code containing variables identified by ConTest. ARC works by using a genetic algorithm without crossover (GA¬C) to evolve variants of an incorrect concurrent Java program into a variant that fixes all known bugs.

Axis \cite{liu2012axis} is a fully automatic bug fixing technique that fix any number of correlated atomicity violations with minimal harm to concurrency by modeling the concurrent properties of a program as Petri nets and using a branch of control theory called the Supervision Based on Place Invariants.

